Bidirectional Tree-Structured LSTM with Head Lexicalization

Sequential LSTM has been extended to model tree structures, giving competitive results for a number of tasks. Existing methods model constituent trees by bottom-up combinations of constituent nodes, making direct use of input word information only for leaf nodes. This is different from sequential LSTMs, which contain reference to input words for each node. In this paper, we propose a method for automatic head-lexicalization for tree-structure LSTMs, propagating head words from leaf nodes to every constituent node. In addition, enabled by head lexicalization, we build a tree LSTM in the top-down direction, which corresponds to bidirectional sequential LSTM structurally. Experiments show that both extensions give better representations of tree structures. Our final model gives the best results on the Standford Sentiment Treebank and highly competitive results on the TREC question type classification task.

==> latex/relatedwork1.tex <==
\textbf{LSTM} Recurrent neural network (RNN) \cite{elman1990finding,mikolov2010recurrent} achieves success on modeling linear structures due to its ability to preserve history information over arbitrary length sequences. 
RNN decides its hidden state based on both the current input and a previous hidden state.  
In theory, it can carry over unbounded history information. 
Long Short-Term Memory (LSTM) \cite{hochreiter1997long} is a special type RNN that leverages multiple gate vectors and a memory cell vector to 
solve the vanishing  and exploding gradient problems of training RNNs. 
%LSTM has strong representation power and can encode complicated sequences into low-dimensional, real-valued vectors. 
It  has been successfully applied to parsing \cite{vinyals2015grammar}, 
sentiment classification \cite{tai15,li2015tree}, speech recognition \cite{graves2013hybrid}, 
machine translation \cite{sutskever2014sequence,bahdanau2014neural} and image captioning \cite{vinyals2015show}.
There are many variants of sequential LSTMs, such as simple Gated Recurrent Neural Networks \cite{cho-EtAl:2014:SSST-8}. 
\newcite{greff2015lstm} compared various architectures of LSTM.  In this paper, we take the standard LSTM with peephole connections \cite{gers2000recurrent} as a baseline. 


\textbf{Structured LSTM extensions} There has been a line of research that extends the standard sequential LSTM in order to model more complex structures.
\newcite{DBLP:journals/corr/KalchbrennerDG15} proposed  Grid LSTM to process multi-dimensional data. 
\newcite{theis2015generative} proposed Spatial LSTM  to handle image data. 
\newcite{dyer-EtAl:2015:ACL-IJCNLP} designed Stack LSTM by adding a top pointer into sequential LSTM to deal with \emph{push} and \emph{pop} sequences of a stack. 
\newcite{tai15}, \newcite{zhu15} and \newcite{le15} extended sequential LSTM to Tree-Structured LSTM (\textbf{Tree LSTM}) by adding branching factors. 
Experiments demonstrated that Tree LSTM can outperform competitive LSTM baselines on several tasks, such as semantic relatedness prediction and sentiment classification.  
\newcite{li2015tree} further investigated the effectiveness of Tree LSTM on various tasks and discussed when Tree LSTM is necessary.   
In addition, \newcite{graph} employed graph gated unit to model graph-based structures. 

\textbf{Tree LSTMs} The idea of extending linear recurrent structure to tree recurrent structure is reminiscent of extending Feed-forward Neural Network to Recursive Neural Network (ReNN) \cite{Socher2013EMNLP,le14} to support information flow over trees. 
In addition to \newcite{tai15}, \newcite{zhu15} and \newcite{le15}, who explicitly named their models as Tree LSTMs,  \newcite{cho-EtAl:2014:SSST-8} designed gated recurrent units over tree structures, and \newcite{ChenQZWH15} introduced gate mechanism to recursive neural networks.
These can also be regarded as variants of Tree LSTM. 

Both \newcite{zhu15} and \newcite{le15} proposed \emph{Binary Tree LSTM} models, which can be applied to situations where  there are exactly two children of each internal node in a tree.
The difference between \newcite{zhu15} and \newcite{le15} is that besides using two forget gates, \newcite{le15} also make use of two input gates to let a node know its sibling. 
\newcite{tai15} introduced \emph{Child-Sum Tree LSTM} and \emph{N-ary Tree LSTM}.   
Child-Sum Tree LSTM  can support multiple children, while the N-ary Tree LSTM works only for at most $N$-ary branching trees. 
In this perspective, Binary Tree LSTM is  a special case of N-ary Tree LSTM with $N=2$. 

According to the tree structure, when a Child-Sum Tree LSTM is applied to a dependency tree, it is referred to as \emph{Dependency Tree LSTM}. 
The \emph{Binary Tree LSTM} is also referred to as \emph{Constituent Tree LSTM}.   
Based on \newcite{tai15}, \newcite{bidir}  introduced a Tree LSTM model that can handle different types of children. 
A dependency tree naturally contains lexical information at every node, while  only leaf nodes contain  lexical information in a constituent tree.  
None of these methods \cite{tai15,zhu15,le15} make direct use of lexical input for internal nodes when using constituent Tree LSTMs. 

\textbf{Bi-LSTM} Another common extension to sequential LSTM is to include bidirectional information \cite{graves2013hybrid}, which can models history both left-to-right and right-to-left. 
The aforementioned Tree LSTM models \cite{tai15,zhu15,le15}  propagates history memories of children to their parent in the bottom-up direction only, while  
ignoring the top-down information flow from parent to its children.  \newcite{topdown} proposed  a top-down Tree LSTM to estimate the generation probability of a \emph{dependency} tree. 
However, no corresponding bottom-up Tree LSTM is incorporated into their model.  

\newcite{paulus2014global}  leveraged bidirectional information over recursive binary trees by propagating global belief recursively down from the tree root to leaf nodes. 
However, their model is based on recursive neural network rather than  LSTM. 
The closest in spirit to our method, \newcite{bidir} adopted a bidirectional Tree LSTM model to jointly extract named entities and relations under \emph{dependency} tree structure. 
For \emph{constituent} tree structures, however, their model does not work due to lack of word inputs on non-leaf constituent nodes, and in particular  the root node. 
Our head lexicalization allows us to investigate the top-down constituent Tree LSTM. To our knowledge, we are the first to report a bidirectional constituent Tree LSTM.

